Emergent Communication under Competition

The literature in modern machine learning has only negative results for learning to communicate between competitive agents using standard RL. We introduce a modified sender-receiver game to study the spectrum of partially-competitive scenarios and show communication can indeed emerge in a competitive setting. We empirically demonstrate three key takeaways for future research. First, we show that communication is proportional to cooperation, and it can occur for partially competitive scenarios using standard learning algorithms. Second, we highlight the difference between communication and manipulation and extend previous metrics of communication to the competitive case. Third, we investigate the negotiation game where previous work failed to learn communication between independent agents (Cao et al., 2018). We show that, in this setting, both agents must benefit from communication for it to emerge; and, with a slight modification to the game, we demonstrate successful communication between competitive agents. We hope this work overturns misconceptions and inspires more research in competitive emergent communication.

==> rebuttal.tex <==
We would like to thank the reviewers for their detailed comments and the time they spent reading and reviewing our paper. We are very pleased that reviewers enjoyed the paper and found it well written (R1), and clear and relevant---especially with regard to related work (R1, R2, R3). We appreciate that the reviewers agree that our claims align with our results (R3), and that overall it is an interesting and original contribution (R1, R2, R3) that could attract a lot of attention and discussion (R2). We are happy that reviewers appreciate our efforts for clear research through open-source reproducibility (R1, R2), the methodical approach we take with our research questions (R2), and clear explanation with plots and graphics that are easy to interpret (R1).   

We are glad R1 sees our conclusion as a "nice result" that motivates further research, and R2 found our contribution "truly significant" noting that "might have a strong impact within communities that study the emergence of communication" (especially as we position our work "relative to other contributions"). 

R3's main concern is that our contribution is too light and would benefit from more theory. We can see how our three takeaways may seem "trivial" (R3) in retrospect---especially our first result that communication is inversely proportional to the level of competition in the game. As we point out, this is a known result in classical game theory and also fairly intuitive. However, this makes the contribution even more necessary since no previous work in emergent communication (EC) has looked at their setup from this perspective, nor have they explicitly quantified the level of competition in their games, as we do. Our experiment is not about novel methods or algorithms but advancing the literature by pointing out this missing perspective and demonstrating how to leverage it in contemporary EC research. For this reason, our next takeaways demonstrate (1) how to use this perspective to extend metrics of communication to competitive scenarios, and (2) how an existing game can be modified to learn communication where the previous work has failed to do so.

To this end, we believe the existing theory (Crawford and Sobel, 1982 "Strategic Information Transmission") is sufficient for our goals, so our work is primarily empirical. We agree with R3 that games need to quantify their level of competitiveness and theoretical analysis already exists for many different types of games (e.g. the cooperative-competitive ("coco") value described by Kalai and Kalai (2012, "Cooperation in strategic games revisited")). Still, new games may not fit into existing frameworks. Empirically, we demonstrate that a non-communication baseline is an effective heuristic for determining the degree to which agents benefit from communication. In terms of theory, it would be interesting to formulate an overarching method for evaluating competitiveness in all games; however, this project is beyond the scope of our current analysis. We hope our empirical work helps pave the way for more research in evaluating and measuring competitive communication.

R2 has a different concern about whether our results generalise to more complex communication protocols. We first would like to point out that communication in the negotiation game (Cao et al., 2019 "Emergent Communication through Negotiation") with which we experiment, is fairly standard RNN-based. More complicated protocols generally use the same framework but simply increase the size of the vocabulary. We agree that insights from the models presented earlier in our paper (the circular game) may not generalize as easily to more complex situations because the degree of competitiveness there is clearly specified, and the protocol is relatively simple. Instead, these experiments validate the general idea of competitiveness affecting the level of communication; and, due to the simplicity of our model, we are able to demonstrate this using a precise and highly-controlled setting. Still, some results are very likely to generalize to a more complicated setting---for example, our demonstration that competition-communication is not perfectly linear, even in a simple setting, and that instabilities of RL optimization should be taken into account (e.g. bias = 120,150).

Finally, we have fixed the notation issue (R1), the display-out-of-limit issue (R2), and will be regenerating our graphs to save them in a vectorial format (R2). We thank the reviewers for their careful reading and pointing out these mistakes.


